Neural Ordinary Differential Equations for Nonlinear System Identification

Neural ordinary differential equations (NODE) have been recently proposed as a promising approach for nonlinear system identification tasks. In this work, we systematically compare their predictive performance with current state-of-the-art nonlinear and classical linear methods. In particular, we present a quantitative study comparing NODE's performance against neural state-space models and classical linear system identification methods. We evaluate the inference speed and prediction performance of each method on open-loop errors across eight different dynamical systems. The experiments show that NODEs can consistently improve the prediction accuracy by an order of magnitude compared to benchmark methods. Besides improved accuracy, we also observed that NODEs are less sensitive to hyperparameters compared to neural state-space models. On the other hand, these performance gains come with a slight increase of computation at the inference time.

==> background.tex <==
\section{Background}
\label{sec:background}

Previous works \cite{haber2017stable, tuor2020constrained, chashchin2019predicting, drgona2020spectral} have shown that deep neural networks can be interpreted as Euler discretizations of an underlying dynamical system. As the step size approaches zero, the time-/depth-evolution of the hidden units can be represented as a differential equation (presented below), which can be solved using an ODE solver \cite{chen2018neural}.

\begin{equation}
    \frac{d \mathbf{h_t}}{dt} = \mathbf{f}(\mathbf{h(t)}, t,\theta)
\label{eq:dh_t}
\end{equation}

In eq. \ref{eq:dh_t}, $\mathbf{f}(\mathbf{h(t)}, t,\theta)$ refers to the vector field that is often parmeterized by a neural network. In a neural ordinary differential equation (NODE), the state of a system ($\mathbf{s}(t_1$) can therefore be expressed as :

\begin{align*}
    \mathbf{s}(t_1) &= \mathbf{s}(t_0) + \int_{t_0}^{t_1}  f(\mathbf{s}(t), t,\theta) dt \nonumber\\
                    &= ODESolve(s(t_0), f, t_0, t_1, \theta) 
\end{align*}

At each time $t$, the state values $\mathbf{s}(t+1)$ of the next timestep $t+1$ can therefore be forecasted using an off-the-shelf ODE solver. The parameters $\theta$, used to define the vector field $f$, can be computed using the adjoint sensitivity method \cite{pontryagin1987mathematical, chen2018neural}.

The NODE formulation can be particularly suitable for system identification tasks, as real-world phenomena are mostly continuous-time evolution processes (which are often unknown) that generate continuous observations; and as such, a predictive model to forecast future behavior should consider temporal integration methods that are typically used to solve ODEs \cite{alvarez2020}. Indeed, NODEs are only beginning to be deployed in system identification tasks \cite{greydanus2019hamiltonian, cranmer2020lagrangian, alvarez2020, cranmer2020lagrangian}. However, there still remains a research need to benchmark the performance of NODEs against current state-of-the-art state-space models for a diverse range of dynamical systems. 
